VDKMS: Vehicular Decentralized Key Management System for Cellular Vehicular-to-Everything Networks, A Blockchain-Based Approach

The rapid development of intelligent transportation systems and connected vehicles has highlighted the need for secure and efficient key management systems (KMS). In this paper, we introduce VDKMS (Vehicular Decentralized Key Management System), a novel Decentralized Key Management System designed specifically as an infrastructure for Cellular Vehicular-to-Everything (V2X) networks, utilizing a blockchain-based approach. The proposed VDKMS addresses the challenges of secure communication, privacy preservation, and efficient key management in V2X scenarios. It integrates blockchain technology, Self-Sovereign Identity (SSI) principles, and Decentralized Identifiers (DIDs) to enable secure and trustworthy V2X applications among vehicles, infrastructures, and networks. We first provide a comprehensive overview of the system architecture, components, protocols, and workflows, covering aspects such as provisioning, registration, verification, and authorization. We then present a detailed performance evaluation, discussing the security properties and compatibility of the proposed solution, as well as a security analysis. Finally, we present potential applications in the vehicular ecosystem that can leverage the advantages of our approach.

==> protocols/full.tex <==
\begin{figure}
\protocol{Proof of Publication of $m$ between verifier $\enclaveparty$ and prover $\ekdparty$ } 
{\\
\underline{Parameters:} \\
$n_c$: publication of $m$ needs at least $n_c$ confirmation \\
$CB:$ a recent checkpoint block \\
$\delta(CB)$: difficulty of $CB$ \\
$\tau$: expected block interval of main chain \\
$\epsilon$: slackness factor\\[2mm]
\underline{\bf Verifier $\enclaveparty$ (a contract \tee):} \\
$t_1\gets$ \tee.timer() \\
$r \sample \bin^{\secpar}$ \\
send $(m,r)$ to $\ekdparty$ \\
receive $\pi_{(m,r)}=(CB, B_1, \cdots, B_n)$ from $\ekdparty$ \\
$t_2\gets$ \tee.timer() \\
\pcif $\pi_{(m,r)}$ is not a valid chain, output $\false$ \\
let $B_i \in \pi_{(m,r)}$ be the block that contains $(m,r)$, output $\false$ if $\nexists B_i$ \\
\pcif $B_i$ has less than $n_c$ confirmation, i.e. $n-i < n_c$, output $\false$ \\
\pcif any $B\in \pi_{(m,r)}$ has a lower difficulty than $\delta(CB)$, output $\false$ \\
\pcif $t_2 - t_1 < (n-i)\times \tau \times \epsilon$: output $\true$ and update checkpiont $CB=B_n$ \\
\pcelse: output $\false$ \\[2mm]
\underline{\bf Prover $\ekdparty$:} \\
\onrecv $(m,r)$ from $\enclaveparty$: \\
\t send $(m,r)$ to the blockchain, denote the including block $B_i$ \\
\t send a subchain from $CB$ to $B_{i+n_c}$ (inclusive) to $\enclaveparty$
}
\caption{Proof of Publication}
\label{fig:proofofpublication}
\end{figure}
